CayleyNets: Graph Convolutional Neural Networks with Complex Rational Spectral Filters

The rise of graph-structured data such as social networks, regulatory networks, citation graphs, and functional brain networks, in combination with resounding success of deep learning in various applications, has brought the interest in generalizing deep learning models to non-Euclidean domains. In this paper, we introduce a new spectral domain convolutional architecture for deep learning on graphs. The core ingredient of our model is a new class of parametric rational complex functions (Cayley polynomials) allowing to efficiently compute spectral filters on graphs that specialize on frequency bands of interest. Our model generates rich spectral filters that are localized in space, scales linearly with the size of the input data for sparsely-connected graphs, and can handle different constructions of Laplacian operators. Extensive experimental results show the superior performance of our approach, in comparison to other spectral domain convolutional architectures, on spectral image classification, community detection, vertex classification and matrix completion tasks.

==> figures/community_detection/ChebNet_CayleyNet_val_test_comparison_constant_signals_high_var_order_long_run_cap_size2.tex <==
% This file was created by matplotlib2tikz v0.6.7.
\begin{tikzpicture}[font=\fontsize{6}{8} \selectfont]

\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
%title={Validation Accuracy},
xlabel={\small Order $r$},
ylabel={\small Accuracy \%},
xmin=0.4, xmax=13.6,
ymin=20.5000005042553, ymax=104.642857118845,
ylabel shift = -5 pt,
xlabel shift = -2pt,
width=\fwidth,
height=\fheight,
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black},
legend style={draw=white!80.0!black, font=\small, inner sep=1pt},
legend cell align={left},
legend entries={{CayleyNet},{ChebNet}},
legend pos = south east
%legend style={at={(0.5,1.325)}, anchor=north,legend columns=-1}
]

\addplot [semithick, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 90.142855834961
3 96.2285704040527
5 97.2571417999268
7 98.0571421051025
9 98.4571424102783
11 98.8285707092285
13 99.1428567504883
};
\addplot [semithick, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 32.3142863464356
3 37.7000006008148
5 63.1285716629028
7 74.2142859077454
9 80.6428559494018
11 85.4285704040527
13 86.9142839431763
};

\path [draw=color0, semithick] (axis cs:1,89.6277771629404)
--(axis cs:1,90.6579345069815);

\path [draw=color0, semithick] (axis cs:3,95.7759138587851)
--(axis cs:3,96.6812269493204);

\path [draw=color0, semithick] (axis cs:5,96.6688204729781)
--(axis cs:5,97.8454631268754);

\path [draw=color0, semithick] (axis cs:7,97.3625564601836)
--(axis cs:7,98.7517277500215);

\path [draw=color0, semithick] (axis cs:9,98.0490608308123)
--(axis cs:9,98.8652239897444);

\path [draw=color0, semithick] (axis cs:11,98.400952610021)
--(axis cs:11,99.256188808436);

\path [draw=color0, semithick] (axis cs:13,98.9408261490946)
--(axis cs:13,99.3448873518819);

\path [draw=color1, semithick] (axis cs:1,31.1753645713642)
--(axis cs:1,33.453208121507);

\path [draw=color1, semithick] (axis cs:3,35.9405364529497)
--(axis cs:3,39.4594647486799);

\path [draw=color1, semithick] (axis cs:5,61.051043615415)
--(axis cs:5,65.2060997103907);

\path [draw=color1, semithick] (axis cs:7,72.873786750862)
--(axis cs:7,75.5547850646288);

\path [draw=color1, semithick] (axis cs:9,78.9462207987082)
--(axis cs:9,82.3394911000955);

\path [draw=color1, semithick] (axis cs:11,84.2248347823174)
--(axis cs:11,86.6323060257881);

\path [draw=color1, semithick] (axis cs:13,85.6490499742799)
--(axis cs:13,88.1795179120726);

\addplot [semithick, color1, mark=-, mark size=5, mark options={solid}, only marks]
table {%
1 89.6277771629404
3 95.7759138587851
5 96.6688204729781
7 97.3625564601836
9 98.0490608308123
11 98.400952610021
13 98.9408261490946
};

\addplot [semithick, color1, mark=-, mark size=5, mark options={solid}, only marks]
table {%
1 90.6579345069815
3 96.6812269493204
5 97.8454631268754
7 98.7517277500215
9 98.8652239897444
11 99.256188808436
13 99.3448873518819
};

\addplot [semithick, color0, mark=-, mark size=5, mark options={solid}, only marks]
table {%
1 31.1753645713642
3 35.9405364529497
5 61.051043615415
7 72.873786750862
9 78.9462207987082
11 84.2248347823174
13 85.6490499742799
};
\addplot [semithick, color0, mark=-, mark size=5, mark options={solid}, only marks]
table {%
1 33.453208121507
3 39.4594647486799
5 65.2060997103907
7 75.5547850646288
9 82.3394911000955
11 86.6323060257881
13 88.1795179120726
};

\end{axis}

\end{tikzpicture}
